Latent Bandits Revisited

A latent bandit problem is one in which the learning agent knows the arm reward distributions conditioned on an unknown discrete latent state. The primary goal of the agent is to identify the latent state, after which it can act optimally. This setting is a natural midpoint between online and offline learning---complex models can be learned offline with the agent identifying latent state online---of practical relevance in, say, recommender systems. In this work, we propose general algorithms for this setting, based on both upper confidence bounds (UCBs) and Thompson sampling. Our methods are contextual and aware of model uncertainty and misspecification. We provide a unified theoretical analysis of our algorithms, which have lower regret than classic bandit policies when the number of latent states is smaller than actions. A comprehensive empirical study showcases the advantages of our approach.

==> extensions.tex <==
\section{Extensions}

\subsection{Changing Latent State}

In non-stationary environments, Garivier et. Moulines proposed two passive adaptations to the UCB algorithm: discounting past observations, or ignoring them completely via a sliding window. We consider the latter, but the former can be similarly analyzed.

Let us define $N_{t+1}(\tau, s) = \sum_{\ell = t - \tau + 1}^t \mathbbm{1}[S_\ell = s]$ as the number of times $s$ was chosen within the $\tau$ most recent rounds, and 
    $$\hat{F}_{t+1}(\tau, s) \leftarrow N_{t+1}(\tau, s)^{-1} \sum_{\ell = t - \tau + 1}^t \mathbbm{1}[S_\ell = s] (\mu_s(A_\ell, X_\ell) - R_\ell),$$
as the empirical average difference between expected and realized reward for choosing latent state $s$ among the most recent rounds.

We propose the following UCB algorithm for nonstationary environments. Initialize $\hat{F}_1(\tau, s) = 0$ for each $s \in S$, and window length $\tau > 0$. For each round $t = 1, 2, \hdots,$
\begin{enumerate}
    % \item $\mu_t(a) \leftarrow$ average reward for arm $a$ up to round $t$.
    \item $C_t \leftarrow \left\{s \in S: \hat{F}_t(\tau, s) < C\sqrt{\frac{\log \min\{\tau, t\}}{N_t(\tau, s)}} \right\}$. 
    \item Observe context $X_t$. For each action $a \in A$, compute
    $$U_t(a) \leftarrow \max_{s \in C_t} \, \mu_s(X_t, a).$$
    \item Select action $A_t \leftarrow \arg\max_{a \in A} U_t(a)$. Let $S_t$ be the corresponding latent state, and $R_t$ the observed reward.
\end{enumerate}
To simplify analysis, we first assume a perfect model with independent arms, though extending to include context and an imperfect model are straightforward using the same techniques as for a fixed latent state. 

Let $s_{t, *}$ and $a_{t, *}$ denote the true latent state and optimal arm for round $t$, and let $B$ be the number of breakpoints, or rounds where the latent state switches. Finally, let $\mathcal{T}$ denote all rounds $t$ such that all rounds $\ell \in [t - \tau + 1, t]$ satisfy $s_{\ell, *} = s_{t, *}$. This includes all rounds that are not too close to a breakpoint. 

We have that the first term in the regret is bounded by,
\begin{align*}
    \sum_{t=1}^T \E{}{\mu_t(a_{t, *}) - U_t(a_{t, *})}
    &\leq C B \tau + \sum_{t \in \mathcal{T}} P(\mu_t(a_{t, *}) \geq U_t(a_{t, *})) \\
    &\leq C B \tau + C \sum_{t \in \mathcal{T}} P(s_{t, *} \not\in C_t),
\end{align*}
where we ignore the rounds too close to breakpoints because the upper-confidence estimates are biased.

For $t \in \mathcal{T}$, and $S_t = s_{t, *}$, we know that $\E{}{\mu_{S_t}(A_t, X_t) - R_t} = \E{}{\mu_t(A_t) - R_t} = 0$.
We have,
\begin{align*}
    P\left(\hat{F}_t(\tau, s_{t, *}) \geq C\sqrt{\frac{\log \min\{t, \tau\}}{N_t(\tau, s_{t, *})}} \right) 
    &\leq \exp\left(-\frac{2N_t(s_{t, *})\left(C\sqrt{\frac{\log \min\{t, \tau\}}{N_t(\tau, s_{t, *})}}\right)^2}{C^2}\right)
\end{align*}
So, the first term can be bounded yielding $P(s_{t, *} \not\in C_t) \leq \frac{1}{\min\{t, \tau\}^2}$. We have that,
\begin{align*}
    \sum_{t \in \mathcal{T}}P(s_{t, *} \not\in C_t) 
    \leq \sum_{t = 1}^{\tau} \frac{1}{t^2} + \sum_{t = \tau + 1}^T \frac{1}{\tau^2}
    \leq \frac{\pi^2}{6} + \left\lceil\frac{T}{\tau^2}\right\rceil
\end{align*}

Now, we have for the second term,
\begin{align*}
    &\sum_{t =1}^T \E{}{U_t(A_t) - \mu_t(A_t)} \\
    &\qquad\leq C  \sum_{t =1}^T \sum_{s \neq s_{t, *}} P(S_t = s) \\
    &\qquad\leq C B \tau + \sum_{t \in \mathcal{T}} \sum_{s \neq s_{t, *}} P(s_{t, *} \not\in C_t) +
    C \sum_{t \in \mathcal{T}} \sum_{s \neq s_{t, *}} P(s_{t, *} \in C_t) P(S_t = s \mid s_{t, *} \in C_t)
\end{align*}
The term involving $P(s_{t, *} \not\in C_t)$ can be bounded using the same analysis as above. 

Let $1 = t_0 < t_1 < \hdots < t_{B} < t_{B + 1} = T$ be the rounds for the $B$ breakpoints. We can write,
\begin{align*}
    &\sum_{t \in \mathcal{T}} \sum_{s \neq s_{t, *}} P(s_{t, *} \in C_t) P(S_t = s \mid s_{t, *} \in C_t) \\
    &\qquad = \sum_{b = 0}^B \sum_{t = t_b}^{t_{b+1} - 1} \sum_{s \neq s_{t, *}} P(s_{t, *} \in C_t) P(S_t = s \mid s_{t, *} \in C_t) 
\end{align*}
For any stationary segment $b$, let $s_{b, *}$ be the true latent state, and $a_{b, *}$ be the optimal arm. Also, define $\Delta_{b, a}$ as the suboptimality gap of arm $a$ in the stationary segment.

For round $t \in [t_b, t_{b+1} - 1]$, if $s_{b, *} \in C_t$ and $S_t \neq s_{b, *}$, we notice that,
\begin{align*}
   \E{}{U_t(A_t) - R_t}  
   \geq \mu_t(a_{t, *}) - \mu_t(A_t) = \Delta_{b, A_t}.
\end{align*}
This is because, when arms are independent, only the best arm under a latent state will be pulled. 

Using this, we see that for $s \neq s_{t, *}$, $\hat{F}_t(\tau, s)$ is the sum of random variables with mean at least $\Delta_{b, A_t}$. From this, we can conclude that,
\begin{align*}
     P\left(\hat{F}_t(\tau, s) < C\sqrt{\frac{\log \min\{t, \tau\}}{N_t(\tau, s)}}  \right)
    %  &\leq P\left((1/t)\sum_{t'=1}^t R_{t'} - \mu(A_t) \geq \Delta_{A_t} - \tau \right) \\
     &\leq \exp\left(-\frac{2 N_t(\tau, s) \left(\Delta_{b, A_t} - C\sqrt{\frac{\log \min\{t, \tau\}}{N_t(\tau, s)}} \right)^2}{C^2}\right).
\end{align*}
We see that once $N_t(\tau, s) \geq \frac{2C^2 \log \tau}{\Delta_{b, A_t}^2}$, then we have $C\sqrt{\frac{\log \min \{t, \tau\}}{N_t(\tau, s)}} \leq \frac{\Delta_{b, A_t}}{2}$, and
\begin{align*}
     P\left(\hat{F}_t(\tau, s) < C\sqrt{\frac{\log \min\{t, \tau\}}{N_t(\tau, s)}}  \right)
    %  &\leq P\left((1/t)\sum_{t'=1}^t R_{t'} - \mu(A_t) \geq \Delta_{A_t} - \tau \right) \\
     &\leq \frac{1}{\tau}
\end{align*} 
So once a suboptimal latent state $S_t \neq s_*$ is played $O\left(\frac{\log \tau}{\Delta_{b, A_t}}\right)$ times, it gets ruled out with high probability. 

Let $a_{s, *} = \max_{a \in A} \mu_s(a)$; then whenever $S_t = s$, we know that $A_t = a_{s, *}$. Using the above, we can bound, for $s \neq s_*$,
\begin{align*}
    \sum_{t = t_b}^{t_{b+1} - 1}  P(S_t = s \mid s_* \in C_t)
    &\leq \sum_{t = t_b}^{t_{b+1} - 1}  P\left(s \in C_t \mid \mu_s(a_{s, *}) \geq \mu(a_*) \right) \\
    &\leq \left\lceil\frac{t_{b+1} - t_b}{\tau}\right\rceil + \frac{2C^2 \log \tau}{\Delta_{b, a_{b, *}}^2}
\end{align*}
Combining yields the total regret,
\begin{align*}
    R(T; \pi^U, \theta)
    &\leq \sum_{t=1}^T \E{}{\mu(a_*) - U_t(a_*)} + \sum_{t=1}^T \E{}{U_t(A_t) - \mu(A_t)} \\
    &\leq 2CB\tau  + C \left[\frac{\pi^2}{6} 
    + \sum_{s \in S} \left(\frac{\pi^2}{6} + \left\lceil\frac{T}{\tau^2}\right\rceil 
    + \left\lceil\frac{T}{\tau}\right\rceil 
    + \frac{2C^2 \log \tau}{\Delta_{a_{s, *}}^2} \right) \right].
\end{align*}
